Learning Any-View 6DoF Robotic Grasping in Cluttered Scenes via Neural Surface Rendering

A significant challenge for real-world robotic manipulation is the effective 6DoF grasping of objects in cluttered scenes from any single viewpoint without the need for additional scene exploration. This work reinterprets grasping as rendering and introduces NeuGraspNet, a novel method for 6DoF grasp detection that leverages advances in neural volumetric representations and surface rendering. It encodes the interaction between a robot's end-effector and an object's surface by jointly learning to render the local object surface and learning grasping functions in a shared feature space. The approach uses global (scene-level) features for grasp generation and local (grasp-level) neural surface features for grasp evaluation. This enables effective, fully implicit 6DoF grasp quality prediction, even in partially observed scenes. NeuGraspNet operates on random viewpoints, common in mobile manipulation scenarios, and outperforms existing implicit and semi-implicit grasping methods. The real-world applicability of the method has been demonstrated with a mobile manipulator robot, grasping in open, cluttered spaces. Project website at https://sites.google.com/view/neugraspnet

==> RSS/sec/2_background.tex <==
\section{Background}

\subsection{Problem description}\label{subsec:problem}
In a cluttered scene with $M$ objects placed on a support surface, we are given a 3D pointcloud of $N$ points $\mathbf{x} \in \mathbb{R}^3$ captured by a depth camera. The camera is pointed towards the objects but can be placed at an arbitrary viewing angle and distance, i.e., the viewpoint is on the S$^2$ sphere with an arbitrary sphere radius $\mathbf{rad} \in \mathbb{R}$. Most grasping methods consider a robot equipped with a two-fingered gripper. Formally, a grasp pose $\mathbf{g} \in \mathbb{R}^6$ can be represented as an approaching 6-dimensional vector (3D positions and orientations) in the SE(3) space from the center of the robotic gripper's center to a point on the surface of an object. Thus, 6DoF grasping can be defined as the problem of using the scene information $\mathbf{x}$ to detect SE(3) grasp poses $\mathbf{g}$ likely to achieve grasp success. The likelihood of success of a grasp is interpreted as the grasp's quality $q \in [0,1]$.%The overall setting can be viewed as a fully implicit representation learning problem. 

\subsection{Convolutional Occupancy Networks}\label{subsec:convonets}
Convolutional Occupancy Networks (ConvONets)~\cite{Peng2020} are implicit neural representations for learning-based 3D scene reconstruction. Given a pointcloud $\mathbf{x}$ or 3D voxel grid of the scene, ConvONet encodes the scene in a feature space $\psi(\mathbf{x})$ using convolutional encoders which combine global and local scene information. For a query 3D point $\mathbf{p} \in \mathbb{R}^3$, it then predicts the probability of the point $\mathbf{p}$ being occupied using the corresponding feature vector $\psi(\mathbf{x}, \mathbf{p})$. The feature vector is passed through a fully connected decoder network $f_\theta$ with a sigmoid at the output leading to the occupancy prediction $o(\mathbf{p}) = f_\theta(\psi(\mathbf{x}, \mathbf{p})) \to [0,1]$. ConvONets combine convolutional encoders with implicit occupancy decoders, effectively leveraging spatial inductive biases, i.e., exploiting the global feature representation capability of CNNs and the fine-grained local geometric modeling capacity of occupancy networks \cite{Mescheder2019}.

\subsection{Surface Rendering} \label{subsec:surfrender}
Neural surface rendering approaches~\cite{niemeyer2020differentiable,Oechsle2021,Wang2021} employ learned implicit geometric representations, such as occupancy networks~\cite{Mescheder2019} or surface models~\cite{Park2019,Wang2021}, to render realistic 3D object surfaces. While some learned geometric representations require explicit 3D supervision~\cite{Mescheder2019,Park2019,Peng2020}, advances in neural radiance fields~\cite{Mildenhall2020} and surface model learning have also enabled the reconstruction of accurate geometry from multi-view 2D images only~\cite{niemeyer2020differentiable,Wang2021}. Given any implicit geometric representation that can predict the occupancy probability $o(\mathbf{p}) \in [0,1]$ of a point $\mathbf{p}$ in the scene, the surface is implicitly determined by the level set $o(\mathbf{p}) = 0.5$, i.e., the transition between occupied and unoccupied space. The surface points can be extracted at an arbitrary resolution using either isosurface extraction techniques~\cite{Mescheder2019} or by ray-marching from a virtual camera pose~\cite{niemeyer2020differentiable,Oechsle2021}.%s with some intrinsic camera matrix $C$ spawned at different poses $\mathbf{p}_{c_k}$ towards the scene. Each camera +++

==> structure.tex <==
Name: 

NGD= Neural Grasp Detection
NGF = Neural Grasping Fields (maybe it exists?)
6D-NeuGrasp (neu = new in german) -- favorite
6D-NeuGraspNet ?


Motivation:
6D grasping is hard (harder than just top down)
6D grasping in clutter is even harder
6D grasping in clutter with only a single partial view is verrry hard
It has been shown that 3D scene reconstruction can help grasping (GIGA).
SOTA for 3D scene reconstruction is typically through implicit occupancy/SDF networks.
Our assumption is that for every 6D grasp, the key features are of those 3D points that define the surface that the grasp will "interact" with. We use neural surface rendering to select these key 3D points and train a network that can back-prop through the features of these points. This allows end-to-end training and feature extraction of pointsets relevant to each grasp.
Crucially, our method also works for "unseen" parts of the scene through shape completion from partial views.
We also propose using an SO(3) equivariant encoder/decoder that is equivariant to rotations of the grasps.

Method:
3D reconstruction: occupancy network
Grasp sampling: GPG
Neural surface rendering
local SDF loss
SE3-group grasp representation
SE3 encoder for occupancy
SO3 - VN for local points
Overall network

Figures:
- Overall network architecture
- The grasp rendering (For each grasp, where the camera is and how it selects the surface points)
- Grasp candidates, good and bad grasp visualization, shape completion
- "Unseen" area grasp generation/selection
- Real robot experiment: YCB objects + random everyday objects

losses
grasp evaluation: sampling and inference
Exp:
Dataset generation
Training
Hyperparams
Network details

Success Rates:
Single object scenes
Multiple Object scenes
New arrangement of seen objects
New arrangement of new objects

Shape completion results and comparison with GIGA

Ablations:
6D GIGA (No rendering)
SDF (with and without)
Random grasps vs GPG sampling
SO/E(3) Equivariance at grasp level and at scene level...

Comparisons with implicit baselines:
VGN (implicit in 3D)
GIGA (implicit in 3D)
PointNetGPD (implicit in 6D)
+++

